Towards Lifelong Dialogue Agents via Timeline-based Memory Management

To achieve lifelong human-agent interaction, dialogue agents need to constantly memorize perceived information and properly retrieve it for response generation (RG). While prior studies focus on getting rid of outdated memories to improve retrieval quality, we argue that such memories provide rich, important contextual cues for RG (e.g., changes in user behaviors) in long-term conversations. We present THEANINE, a framework for LLM-based lifelong dialogue agents. THEANINE discards memory removal and manages large-scale memories by linking them based on their temporal and cause-effect relation. Enabled by this linking structure, THEANINE augments RG with memory timelines - series of memories representing the evolution or causality of relevant past events. Along with THEANINE, we introduce TeaFarm, a counterfactual-driven evaluation scheme, addressing the limitation of G-Eval and human efforts when assessing agent performance in integrating past memories into RG. A supplementary video for THEANINE and data for TeaFarm are at https://huggingface.co/spaces/ResearcherScholar/Theanine.

==> tables/g_eval_new.tex <==
\begin{table}[!t]
\centering
\resizebox{0.85\columnwidth}{!}{
\begin{tabular}{@{}lc@{}}
\toprule
% & \multicolumn{2}{c}{\textbf{Success Rate (SR; \%)}}\\ \cmidrule(l){2-3}
\textbf{Construction Methods} & \textbf{Retrieve Helpful Memories} \\ 
\midrule
List (Memory Retrieval)             & 00.00\%  \\
\, + Memory Update$^*$           & 00.00\% \\
Rsum-LLM$^*$                     & N/A (no retrieval) \\
MemoChat$^*$                     & 00.00\%  \\
COMEDY$^*$                       & 00.00\%  \\
\cellcolor{brown!14}\tealeaf\textbf{\theanine} (Ours)        & \cellcolor{brown!14}\textbf{00.00\%} \\ 
\bottomrule
\end{tabular}%
}
\caption{G-Eval on how memory construction affects retrieval quality. We report the success rate (SR; \%).}
\label{tab:g_eval_new}
\end{table}\textbf{}


% \begin{table}[!t]
% \centering
% \resizebox{1\columnwidth}{!}{
% \begin{tabular}{@{}lcc@{}}
% \toprule
% % & \multicolumn{2}{c}{\textbf{Success Rate (SR; \%)}}\\ \cmidrule(l){2-3}
% \textbf{Methods} & \textbf{Correctly Recall} & \textbf{Not Contradict the Past} \\ 
% \midrule
% All History                     & 00.00 & 00.00 \\
% All Memories \& $\mathcal{D}$    & 00.00 & 00.00 \\
% \, + Memory Update$^*$           & 00.00 & 00.00 \\
% Memory Retrieval                 & 00.00 & 00.00 \\
% \, + Memory Update$^*$           & \textbf{00.00} & \textbf{00.00} \\
% Rsum-LLM$^*$                     & 00.00 & 00.00 \\
% MemoChat$^*$                     & 00.00 & 00.00 \\
% COMEDY$^*$                       & 00.00 & 00.00 \\
% \textbf{\theanine} (Ours)        & 00.00 & 00.00 \\ 
% \midrule
% w/o Relation-aware Linking                   & 00.00 & 00.00 \\
% w/o Timeline Refinement                & \textbf{00.00} & \textbf{00.00} \\
% \bottomrule
% \end{tabular}%
% }
% \caption{G-eval results.}
% \label{tab:g_eval_new}
% \end{table}\textbf{}
